Segmentation-driven 6D Object Pose Estimation

The most recent trend in estimating the 6D pose of rigid objects has been to train deep networks to either directly regress the pose from the image or to predict the 2D locations of 3D keypoints, from which the pose can be obtained using a PnP algorithm. In both cases, the object is treated as a global entity, and a single pose estimate is computed. As a consequence, the resulting techniques can be vulnerable to large occlusions. In this paper, we introduce a segmentation-driven 6D pose estimation framework where each visible part of the objects contributes a local pose prediction in the form of 2D keypoint locations. We then use a predicted measure of confidence to combine these pose candidates into a robust set of 3D-to-2D correspondences, from which a reliable pose estimate can be obtained. We outperform the state-of-the-art on the challenging Occluded-LINEMOD and YCB-Video datasets, which is evidence that our approach deals well with multiple poorly-textured objects occluding each other. Furthermore, it relies on a simple enough architecture to achieve real-time performance.

==> fig/occlinemod_2dRes-crop.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
	\centering
	\includegraphics{./fig/occlinemod_2dRes-crop.pdf}
	\caption{Running.}
	\label{fig:occlinemod_2dres}
\end{figure*}
 


==> fig/ransac.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure}
\centering
\begin{subfigure}{0.4\linewidth} % width of right subfigure
	\includegraphics[width=\linewidth]{fig/bigpicture/seg.png}
	\caption{DNC} % subcaption
\end{subfigure}
\hspace{10pt}
\begin{subfigure}{0.4\linewidth} % width of left subfigure
	\includegraphics[width=\linewidth]{fig/bigpicture/image.png}
	\caption{RNC} % subcaption
\end{subfigure}
\caption{Effect of weighted RANSAC.}
\label{fig:ransac_demo}
\end{figure}


==> fig/ycbvideo_eval-crop.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{figure*}
	\centering
	\includegraphics{./fig/ycbvideo_eval-crop.pdf}
	\caption{Accuracy of the 21 object classes in REP-5px (top) and ADD-0.1d (bottom) on YCB-Video dataset, respectively.}
	\label{fig:ycbvideo_eval}
\end{figure*}

 


==> table/different_3dpoints.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

\begin{table}
	\centering
	\begin{tabular}{lcccc}
		\hline
		&	8	&	16	&	32	&	64	\\
		\hline
		Ape	& \\
		Can	& \\
		Cat & \\
		Driller	& \\
		Duck	& \\
		Eggbox$^*$	& \\
		Glue$^*$	& \\
		Holepun.	& \\
		\hline
		Average		& \\
	\end{tabular}
	\caption{Effect of different 3D points settings (in REP-5px). Besides the typical way of choose the 8 corners of 3D bounding box of meshes, we directly choose different number of 3D points from the surface of meshes randomly. It works and shows that more points can generate more accurate pose result (see Sec.~\ref{sec:different3Dpoints}).}
	\label{tab:different_3dpoints}
\end{table} 

